RuleR: Improving LLM Controllability by Rule-based Data Recycling

Large language models (LLMs) still lack delicate controllability over their responses, which is critical to enhancing their performance and the user experience. However, curating supervised fine-tuning (SFT) datasets to improve LLM controllability usually relies on human experts or proprietary LLMs, which requires additional costs. To bridge this gap, we propose Rule-based Data Recycling (RuleR), a data augmentation method incorporating multiple constraints into the original data samples according to predefined rules, which creates new training tasks to consolidate the controllability of LLMs. Instead of creating new data from scratch, RuleR "recycles" existing data by simply applying rule-based edits to their responses and appending the rule-instructions in their original instructions. Experimental results demonstrate RuleR's effectiveness in improving LLM controllability while maintaining general instruction-following capabilities.

==> table_rules_2.tex <==
\begin{table*}[ht]
\centering
\small % Adjust font size
\scalebox{0.8}{ % Adjust the scaling factor as needed
\begin{tabular}{p{0.35\columnwidth}|p{0.35\columnwidth}|p{1.2\columnwidth}}
\toprule
\textbf{Instruction Group} & \textbf{Instruction} & \textbf{Description} \\
\midrule
Keywords & Keyword Inclusion & Include the specific word in the response \\
\midrule
Keywords & Keyword Frequency & Include the specific word equal/less/more $N$ times in response\\
\midrule
Keywords & Keyword Type Frequency  & Include the specific word types equal/less/more n times in response \\
\midrule
Length Constraints & Number of Words & The length of the response should equal/less/more $N$ words \\
\midrule
Length Constraints & Number of Sentences & The length of the response should equal/less/more $N$ sentences\\
\midrule
Length Constraints & Number of Paragraphs & The length of the response should equal/less/more $N$ paragraphs \\
\midrule
Detectable Content & Number of Bullet Points  & The response should have exactly/less than/more than $N$ bullet points \\
\midrule
Detectable Content & Keyword Wrapping & Wrap the specific word in the specific format in response \\
\midrule
Detectable Format & Sentence Wrapping & Wrap the specific sentence in the specific format in response \\
\midrule
Detectable Format & Paragraph Wrapping & Wrap the specific paragraph in the specific format in response \\
\midrule
Detectable Format & Bullet Point Wrapping & Wrap the specific bullet point in the specific format in response \\
\midrule
Detectable Format & Instruction Wrapping & Repeat the instruction wrapped in curly brackets first, then provide the response \\
\midrule
Detectable Format & Response Wrapping & The whole response wrapped in curly brackets \\
\midrule
Combination & Instruction Repetition & Repeat the instruction first, then provide the response  \\
\midrule
Combination & Response Repetition & Repeat the same response $N$ times \\
\midrule
Case Change & Uppercase Conversion & The response should all be in uppercase \\
\midrule
Case Change & Lowercase Conversion & The response should all be in lowercase \\
\midrule
Case Change & Letter Uppercase Conversion & The specific letter in response should all be in uppercase\\
\midrule
Case Change & Word Uppercase Conversion & The specific word in response should be in uppercase \\
\midrule
Case Change & Sentence uppercase Conversion & The specific sentence in response should be in uppercase. \\
\midrule
Case Change & Paragraph uppercase Conversion & The specific paragraph in response should be in uppercase\\
\midrule
Punctuation & Selective Punctuation Ignorance & Ignore all specific punctuation in the response \\
\midrule
Punctuation & Complete Punctuation Ignorance & Ignore all punctuation in the response \\
\midrule
Punctuation & Selective Punctuation Replacement & Replace all specific punctuation with new punctuation in the response \\
\midrule
Punctuation & Complete Punctuation Replacement &  Replace all punctuation with new punctuation in the response \\
\bottomrule
\end{tabular}}
\caption{The list of 25 format meta instructions, with brief descriptions. }
\label{tab:list}
\end{table*}
